Data Assimilation: A Mathematical Introduction

These notes provide a systematic mathematical treatment of the subject of data assimilation.

==> chapter5.tex <==
% !TEX root = book.tex
\chapter{Continuous Time: Formulation}\label{sec:ctf}



\section{Set-Up}\label{ssec:csu}

\subsection{Derivation of the Continuous Time Model}


\subsection{Stochastic Integration}


\section{Guiding Examples}\label{ssec:cge}



\section{Smoothing Problem}\label{ssec:csp}


\subsection{Probabilistic Formulation of Data Assimilation}


\subsection{Girsanov Formula}\index{Girsanov formula}




\subsection{Conditional Probabilities}




\subsection{Stochastic Dynamics}


\subsection{Deterministic Dynamics}
\label{ssec:dd202}



\section{Filtering Problem}\label{ssec:cfp}


\section{Illustrations}\label{ssec:cil}






  
\section{Bibliographic Notes}\label{ssec:cbn}




\section{Exercises}
















==> chapter6.tex <==
% !TEX root = book.tex
\chapter{Continuous Time: Smoothing Algorithms}\label{sec:ctsa}

\section{Linear Gaussian Problems: The Kalman-Bucy\index{Kalman-Bucy smoother} Smoother}\label{ssec:kalkal2}


\section{Markov Chain-Monte Carlo Methods}\label{ssec:cmcmc}


\subsection{Deterministic Dynamics}
\label{ssec:dd2c}



\subsection{Stochastic Dynamics}
\label{ssec:sd2c}




\section{Variational Methods}\label{ssec:cvm}



\section{Illustrations}\label{ssec:cil2}



\section{Bibliographic Notes}\label{ssec:cbn2}



\section{Exercises}
\label{sec:exm}




==> chapter7.tex <==
% !TEX root = book.tex
\chapter{Continuous Time: Filtering Algorithms}\label{sec:ctfa}


\section{Linear Gaussian Problems: The Kalman-Bucy Filter}\index{Kalman filter!Kalman-Bucy}\label{ssec:ckbf}


\section{Approximate Gaussian Filters \index{Gaussian filter!approximate}}\label{ssec:cagf}



\subsection{3DVAR\index{3DVAR}}


\subsection{Extended Kalman Filter}\index{Kalman filter!extended}



\subsection{Ensemble Kalman Filter}\index{Kalman filter!ensemble}


\section{The Particle Filter}\label{ssec:cpf}




\section{Large-Time Behaviour of Filters}\label{ssec:csa}

\subsection{The Kalman-Bucy Filter\index{Kalman filter!Kalman-Bucy} in One Dimension}
\label{sssec:kfoc}



 

 
\subsection{The 3DVAR Filter}
\label{sssec:3sc}







\section{Illustrations}\label{ssec:cil3}







\section{Bibliographic Notes}\label{ssec:cbn3}


\section{Exercises}
\label{sec:ex8}



==> chapter8.tex <==
% !TEX root = book.tex
\chapter{Continuous Time: {\sc matlab} Programs} \label{sec:matc}



 
\section{Chapter \ref{sec:ctf} Programs}

\subsection{p1c.m}




\subsection{p2c.m}





\subsection{p3c.m}
\label{ssec:p3c}

\section{Chapter \ref{sec:ctsa} Programs}




\subsection{p4c.m}
\label{ssec:p4c}



\subsection{p5c.m}
\label{ssec:p5c}



\subsection{p6c.m}
\label{ssec:p6c}




\subsection{p7c.m}
\label{ssec:p7c}





\section{Chapter \ref{sec:ctfa} Programs}




\subsection{p8c.m}
\label{ssec:p8c}












%\subsection{p9c.m}
%\label{ssec:p9c}
%
%
%
%\lstinputlisting{./matlab_files/p9c.m}
%\newpage




\subsection{p10c.m}
\label{ssec:p10c}





\subsection{p11c.m}
\label{ssec:p11c}






\subsection{p12c.m}
\label{ssec:p12c}






\subsection{p13c.m}
\label{ssec:p13c}



%






\subsection{p14c.m}
\label{ssec:p14c}







\subsection{p15c.m}
\label{ssec:p15c}



\subsection{p16c.m}
\label{ssec:p16c}

\subsection{p17c.m}
\label{ssec:p17c}

